Noisy UGC Translation at the Character Level: Revisiting Open-Vocabulary Capabilities and Robustness of Char-Based Models

This work explores the capacities of character-based Neural Machine Translation to translate noisy User-Generated Content (UGC) with a strong focus on exploring the limits of such approaches to handle productive UGC phenomena, which almost by definition, cannot be seen at training time. Within a strict zero-shot scenario, we first study the detrimental impact on translation performance of various user-generated content phenomena on a small annotated dataset we developed, and then show that such models are indeed incapable of handling unknown letters, which leads to catastrophic translation failure once such characters are encountered. We further confirm this behavior with a simple, yet insightful, copy task experiment and highlight the importance of reducing the vocabulary size hyper-parameter to increase the robustness of character-based models for machine translation.

==> Intro_Djame.tex <==
%-*- coding: utf-8 -*-
\section{Introduction \label{sec:intro}}

Neural Machine Translation (NMT) models fall far short from being able
to translate noisy User-Generated Content (UGC): the quality of their
translation is often even worse than that of a traditional
phrase-based
system~\cite{DBLP:conf/aclnmt/KhayrallahK18,rosales-nunez-etal-2019-comparison}.
In addition to ambiguous grammatical constructs and the profusion of
ellipsis, the main difficulty encountered when translating UGC is the
high number of out-of-vocabulary tokens (OOVs) resulting from
misspelled words, emoticons, hashtags, mentions and all specific
constructs used in online forums and social medias
\cite{foster:2010:cba,seddahetal:2012:crapbank,eisenstein2013bad,sanguinettietal:2020:treebankingUGC}.
Some of those phenomena can be perceived as noise while the others
are typical markers of language variation among speakers. Moreover,
a certain amount of those same phenomena operate at the lexical
level (either at the character, subword or word levels) \cite{DBLP:journals/corr/abs-2011-02063}. This is why, focusing more on the noise axis, char-based models appear to offer a
natural solution to this  problem~\cite{luong16achieving,ling15character}: indeed these open vocabulary models are designed specifically to address the OOV problem.

In this work, we explore the ability of out-of-the-box character-based
NMT models \cite{DBLP:journals/tacl/LeeCH17_et_al} to address the
challenges raised by UGC translation. While character-based models may
seem promising for such task, to the best of our knowledge, they have
only been tested either on data sets in which noise has been
artificially added through sampling an edited word error data set
\cite{DBLP:conf/iclr/BelinkovB18, ebrahimi18adversarial} and on
canonical data set, in which they prove to be very effective for
translating morphologically-rich languages with a high number of OOV
\cite{luong16achieving}.

However our starting-points experiments show that
character-based systems are outperformed by BPE models even when
translating noisy UGC. To understand this counter-intuitive result, we
conduct several experiments and analysis. In
particular, we  manually annotated 400 sentences at the token
level using a fine grained typology, to perform our
analyses. These sentences correspond to 
worst and the best translated utterances of two MT systems (a char-based and a
transformer-based model). Our results highlight the extreme sensibility of
character-based models to the vocabulary size, a parameter often
overlooked in the literature. Using a simple  set  of experiments we thus
show that these models are unable to perform an {\em easy} copy task due to their
poor handling of unknown and rare characters. By adjusting the
vocabulary size parameter, we drastically improve the robustness of
our character-based model without provoking a large drop in in-domain performance.

Our contributions are as follows:
\begin{itemize}
\item we provide an annotated data set that enables in-depth evaluations
  of the impact of UGC idiosyncrasies;
\item we demonstrate that char-based neural machine translation models are
extremely sensitive to unknown and rare characters on both synthetic 
data and noisy user-generated content;
\item we show how an overlooked hyper-parameter drastically improve char-based MT models
  robustness to natural noise while maintaining in-domain level of
  performance.\draftnote{petit bras non ? -ds} 

\end{itemize}


\iffalse
By analyzing and comparing errors made by our different systems, we
show that (i) char-based neural machine translation models are
extremely sensitive to unknown and rare characters, (ii) contrary to
what was believed, they are not able to translate texts that are
productive in terms of new forms, new structures or domain shifts and
(iii) by drastically limiting their vocabulary size, we can improve
their generalization ability when facing noisy text.
\fi







% \iffalse  
% %%% C'est relou José, on dirait que tu vends des charM







% .....
% to
% explain and characterize challenges posed by these kind of texts, such
% that upcoming works can easily evaluate and develop MT systems that
% are more robust to real-world noise. 

% \draftremove{In order to illustrate our
% approach, we choose to investigate the impact of UGC noise on
% different subword levels.}



% In this regard, char-based models appear to offer a
% natural solution to this
% problem~\cite{luong16achieving,ling15character}: indeed these open
% vocabulary models are designed specifically to address the OOV
% problem. This is why, as part of our comparison, we make use of out-of-the-box character-based
% NMT models \cite{DBLP:journals/tacl/LeeCH17_et_al} to potentially address a range of
% challenges raised by UGC translation. While character-based models may
% seem promising for such task, to the best of our knowledge, they have
% only been tested on either data sets in which noise has been
% artificially added %through sampling an edited word error data set
% \cite{DBLP:conf/iclr/BelinkovB18, ebrahimi18adversarial} or
% canonical data sets, in which they prove to be very effective for
% translating morphologically rich languages with a high number of OOV
% \cite{luong16achieving}.

% However our experiments (\textsection \ref{sec:exp}) show that
% character-based systems are globally outperformed by Byte-pair
% Encoding (BPE) models when translating noisy UGC. \textcolor{red}{In
%   order to understand this counter-intuitive result and derive
%   insights beyond a coarse corpus-level metric, we present our
%   evaluation framework to quantify the impact of noise on translation
%   quality as our main contribution, by including a new data set of
%   noisy UGC in which UGC peculiarities have been manually annotated
%   with their position using a fine-grained typology.% {Mettre plus
%   % l'accent sur le data set si on soumet sur la track Lang Resource and
%   % Evaluation -ds}


% \draftremove{Our contributions can be seen as a negative result as we
% show that character-based NMT models are unable to cope with an ever
% evolving domain with an endless productivity of out-of-vocabulary
% characters.}

% \fi

==> Intro_acl.tex <==
%-*- coding: utf-8 -*-
\section{Introduction  (used for the be arxived paper don't use here)\label{sec:intro}}

Neural Machine Translation (NMT) models fall far short from being able
to translate noisy User-Generated Content (UGC): the quality of their
translation is often even worse than that of a traditional
phrase-based
system~\cite{DBLP:conf/aclnmt/KhayrallahK18,rosales-nunez-etal-2019-comparison}.
In addition to ambiguous grammatical constructs and the profusion of
ellipsis, the main difficulty encountered when translating UGC is the
high number of out-of-vocabulary tokens (OOVs) resulting from
misspelled words, emoticons, hashtags, mentions and all specific
constructs used in online forums and social mediahttps://www.overleaf.com/projects
\cite{foster-2010-cba,seddah-etal-2012-french,eisenstein-2013-bad}.
Some of those phenomena can be perceived as noise while the others
are typical markers of language variations among speakers.  More over,
a certain amount of those same phenomena operate at the character or
at the subword levels, hence the natural question of finding the right
neural architecture and its ideal level of representation to model
both noise and language variation is of crucial importance.

This is why, focusing more on the noise axis, we present in this work
a thorough evaluation of three out-of-the-box NMT architectures
(namely \chartchar, \seqtseq and \transformer) applied to noisy UGC in
a zero-shot scenario. To understand the impact of UGC idiosyncrasies
on translation quality and better understand how these idiosyncrasies
are handled by various neural architecture, we have manually annotated
a parallel corpus of UGC to indicate the position and type of each UGC
idiosyncrasy. We introduced a framework that enables us to generate a
collection of annotated parallel corpora with a dynamic controllable
number of UGC idiosyncrasies and noise types per sentence. Thanks to
our approach, we are able to highlight the `atomic' challenges raised
by each type of UGC as well as the potential complex latent dynamics
between difféerent UGC specificities. While, we focus, in this work,
on machine translation, We believe that the annotated corpus and the
framework we present could be of great interest to perform
fine-grained error analysis for NLP systems dealing with noisy UGC.
  
% Our approach allow us to control the noise types which are present at
% evaluation time by retaining only a subset of the noise occurrences,
% such that the impact on performance can be assessed by removing
% potentially complex latent dynamics between different UGC
% specificities. Those can lead to the intractability of
% individual\draftnote{atomic?} challenges raised by such types of UGC
% idiosyncrasies for NMT.\draftnote{Ce paragraphe est vraiment dur à
%   comprendre, on dirait qu'il est circulaire -ds}


By analyzing and comparing errors made by our different systems using
our typology and data, we illustrate the usefulness of our annotated
collection, as we show evidence that (i) char-based neural machine
translation models are extremely sensitive to unknown and rare
characters, (ii) we noticed advantages over BPE-based models when
translating misspelled words, incorrect tokenization and inconsistent
casing and (iii) by drastically limiting their vocabulary size, we can
improve their generalization ability when facing noisy
text.\draftnote{a revoir, on dirait qu'on vend des cacahuettes, c'est
  relou -ds}


% \iffalse  
% %%% C'est relou José, on dirait que tu vends des charM







% .....
% to
% explain and characterize challenges posed by these kind of texts, such
% that upcoming works can easily evaluate and develop MT systems that
% are more robust to real-world noise. 

% \draftremove{In order to illustrate our
% approach, we choose to investigate the impact of UGC noise on
% different subword levels.}



% In this regard, char-based models appear to offer a
% natural solution to this
% problem~\cite{luong16achieving,ling15character}: indeed these open
% vocabulary models are designed specifically to address the OOV
% problem. This is why, as part of our comparison, we make use of out-of-the-box character-based
% NMT models \cite{DBLP:journals/tacl/LeeCH17_et_al} to potentially address a range of
% challenges raised by UGC translation. While character-based models may
% seem promising for such task, to the best of our knowledge, they have
% only been tested on either data sets in which noise has been
% artificially added %through sampling an edited word error data set
% \cite{DBLP:conf/iclr/BelinkovB18, ebrahimi18adversarial} or
% canonical data sets, in which they prove to be very effective for
% translating morphologically rich languages with a high number of OOV
% \cite{luong16achieving}.

% However our experiments (\textsection \ref{sec:exp}) show that
% character-based systems are globally outperformed by Byte-pair
% Encoding (BPE) models when translating noisy UGC. \textcolor{red}{In
%   order to understand this counter-intuitive result and derive
%   insights beyond a coarse corpus-level metric, we present our
%   evaluation framework to quantify the impact of noise on translation
%   quality as our main contribution, by including a new data set of
%   noisy UGC in which UGC peculiarities have been manually annotated
%   with their position using a fine-grained typology.% {Mettre plus
%   % l'accent sur le data set si on soumet sur la track Lang Resource and
%   % Evaluation -ds}


% \draftremove{Our contributions can be seen as a negative result as we
% show that character-based NMT models are unable to cope with an ever
% evolving domain with an endless productivity of out-of-vocabulary
% characters.}

% \fi

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = ugc_at_charlevel
# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles = Discussion.tex Intro_Djame.tex









#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).tex
	$(TEX) $(latexfile).tex 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
#	bibtex $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
	
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef
	cat $(latexfile).log | grep --text multipl

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: $(latexfile).pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex  & 


up:
	git pull

co:	commit
	
commit:
	git commit -m "update" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up

cp:
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/PapiersEnCours

ebib:
	open $(latexfile).bib


split: bib
	splitappendix $(latexfile).pdf 11
	open -a Skim.app submission.pdf appendix.pdf
	


==> garbage.tex <==
In this work, we aim at exploring the capability of out-of-the-box
character-based NMT models to address the challenges raised by UGC
translation. Because those  character-based models have been specifically designed to
deal with noisy input and to address the problem of translating OOV
tokens, they seem to be a `natural' solution to \draftreplace{the
problem}{some of the main problems} raised by UGC translation.

because of the UGC productivity
(there will always be new forms that will not have been seen during
training), UGC translation requires a model able to learn robust
sentence representations in a zero-shot scenario in which models are
trained from canonical data only. 

In spite of their many promises, to
the best of our knowledge, character-based models have only been
tested either on data sets in which noise has been artificially added
and on canonical data set in which they prove to be very effective for
translating morphologically rich languages with a high number of OOV
words.




%%%% old crap



The contributions of this paper are twofold. First, we evaluate the
performance of character-based methods on two highly noisy natural
corpora of UGC made of French senteces translated into
English. Second, in order to point out and analyze the limits of these
systems, we have manually annotated 400 UGC sentences indicating the
kind of errors/noise they contain, a resource that could be of great
interest to perform fine-grained error analysis for NLP systems
dealing with UGC. By analyzing and comparing errors made by our
systems, we report a negative result showing that character-based
translations are very sensitive to UGC idiosyncrasies and, contrary to
what was believed, are not able to translate texts that are productive
in terms of new forms, new structures or new domains.\footnote{All our
  datasets and systems can be downloaded from
  \url{https://github.com/josecar25/char_based_NMT-noisy_UGC}.}

